What Does the Post-Moore Era Mean for Research Software Engineering?

We are entering the post-Moore era where we no longer enjoy the free ride of the performance growth from simply shrinking the transistor features. However, this does not necessarily mean that we are entering a dark era of computing. On the contrary, sustaining the performance growth of computing in the post-Moore era itself is cutting-edge research. Concretely, heterogeneity and hardware specialization are becoming promising approaches in hardware designs. However, these are paradigm shifts in computer architecture. So what does the post-Moore era mean for research software engineering? This position paper addresses such a question by summarizing possible challenges and opportunities for research software engineering in the post-Moore era. We then briefly discuss what is missing and how we prepare to tackle such challenges and exploit opportunities for the future of computing.

==> license.tex <==
\section*{Government License}

The submitted manuscript has been created by UChicago Argonne, LLC,
Operator of Argonne National Laboratory (“Argonne”). Argonne, a
U.S. Department of Energy Office of Science laboratory, is operated
under Contract No. DE-AC02-06CH11357. The U.S. Government retains for
itself, and others acting on its behalf, a paid-up nonexclusive,
irrevocable worldwide license in said article to reproduce, prepare
derivative works, distribute copies to the public, and perform
publicly and display publicly, by or on behalf of the Government.  The
Department of Energy will provide public access to these results of
federally sponsored research in accordance with the DOE Public Access
Plan. http://energy.gov/downloads/doe-public-access-plan.

